Waveform resampling with LMN method

Resampling is a common technique applied in digital signal processing. Based on the Fast Fourier Transformation (FFT), we apply an optimization called here the LMN method to achieve fast and robust re-sampling. In addition to performance comparisons with some other popular methods, we illustrate the effectiveness of this LMN method in a particle physics experiment: re-sampling of waveforms from Liquid Argon Time Projection Chambers.

==> discussion.tex <==
\appendix{summary of alg}

BOOST: \url{https://www.boost.org/doc/libs/master/libs/math/doc/html/interpolation.html}

Cardinal Cubic B-spline interpolation, 
Cardinal Quadratic B-spline interpolation, 
Cardinal Quintic B-spline interpolation, 
\url{https://en.wikipedia.org/wiki/B-spline} Construction O(n), each call O(1)\\

Whittaker-Shannon interpolation  (very similar to proposed method, Construction O(1), each call O(n) ) \url{https://en.wikipedia.org/wiki/Whittaker%E2%80%93Shannon_interpolation_formula}\\

Cardinal Trigonometric interpolation (use FFT to get coefficients, and then sinc functions) \\


Barycentric Rational Interpolation, Vector-valued Barycentric Rational Interpolation,
(O(N) construction, each call O(n))\\

Catmull-Rom Splines \url{https://en.wikipedia.org/wiki/Centripetal_Catmull%E2%80%93Rom_spline}, (O(logN), using 4 points)\\

Bezier Polynomials  \url{https://en.wikipedia.org/wiki/Bernstein_polynomial}\\

Cubic Hermite interpolation \url{https://en.wikipedia.org/wiki/Cubic_Hermite_spline}, Quintic Hermite interpolation\\
PCHIP interpolation (non-equispaced data, use Cubic Hermite)\\

Modified Akima interpolation , (good for fast varying second derivative) cost same as cubic Hermite\\
Bilinear Uniform Interpolation \url{https://en.wikipedia.org/wiki/Bilinear_interpolation} (2D interpolation)\\ 

EIGEN spline: \url{https://eigen.tuxfamily.org/dox/unsupported/classEigen_1_1Spline.html#:~:text=Detailed%20Description%20template%3Ctypename%20Scalar_%2C%20int%20Dim_%2C%20int%20Degree_%3E,associated%20with%20a%20basis%20function%20C%28u%29%20%3D%E2%88%91i%3D0n%20Ni%2Cp%28u%29Pi}

ROOT: \url{https://root.cern.ch/doc/master/group__Interpolation.html}
LINEAR interpolation;
POLYNOMIAL interpolation, to be used for small number of points since introduces large oscillations;
CSPLINE cubic spline with natural boundary conditions;
CSPLINE\_PERIODIC cubic spline with periodic boundary conditions;
AKIMA, Akima spline with natural boundary conditions ( requires a minimum of 5 points);


SCIPY: \url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.signal.resample_poly.html}

Polyphase: \url{https://www.wavewalkerdsp.com/2021/09/29/polyphase-half-band-filter-for-decimation-by-2/}  contineous data, 

FFT: ... \url{https://github.com/scipy/scipy/blob/v1.11.3/scipy/signal/_signaltools.py#L3036-L3221}

2D Photo: 
